DataSeal: Ensuring the Verifiability of Private Computation on Encrypted Data

Fully Homomorphic Encryption (FHE) allows computations to be performed directly on encrypted data without needing to decrypt it first. This "encryption-in-use" feature is crucial for securely outsourcing computations in privacy-sensitive areas such as healthcare and finance. Nevertheless, in the context of FHE-based cloud computing, clients often worry about the integrity and accuracy of the outcomes. This concern arises from the potential for a malicious server or server-side vulnerabilities that could result in tampering with the data, computations, and results. Ensuring integrity and verifiability with low overhead remains an open problem, as prior attempts have not yet achieved this goal. To tackle this challenge and ensure the verification of FHE's private computations on encrypted data, we introduce DataSeal, which combines the low overhead of the algorithm-based fault tolerance (ABFT) technique with the confidentiality of FHE, offering high efficiency and verification capability. Through thorough testing in diverse contexts, we demonstrate that DataSeal achieves much lower overheads for providing computation verifiability for FHE than other techniques that include MAC, ZKP, and TEE. DataSeal's space and computation overheads decrease to nearly negligible as the problem size increases.

==> contents/definition.tex <==


\begin{definition}[FHE]
A FHE (FHE) scheme is a tuple (KeyGen, Encrypt, Eval, Decrypt) of PPT algorithms:
\begin{itemize}
    \item $KeyGen(1^\lambda,f) \rightarrow (pk,sk, ek)$
    \item $Encrypt_{\text{key}}(x, \tau_x) \rightarrow (c_x)$ where key is either $pk$ or $sk$
    \item $Eval_{pk}(c_x) \rightarrow (c_y)$ where $y = f(x)$
    \item $Decrypt_{key}(c_y) \rightarrow y$
    \item $Decode(y) \rightarrow \tau_y$
\end{itemize}
\end{definition}

\begin{definition}[Dataseal Verification]
A dataseal verifiable FHE (vFHE) scheme is a tuple (KeyGen, Encode Decode, Verify) of PPT algorithms:
\begin{itemize}
    \item $KeyGen(1^\lambda,f) \rightarrow (pk,sk, ek)$
    \item $Encode_{\text{key}}(x) \rightarrow (\tau_x)$ where the key is a secret encoding key (ek)
    \item $Decode(y) \rightarrow \tau_y$
    \item $Verify_{ek}(y, \tau_y) \rightarrow b$, the client accepts if $b = 1$ and rejects otherwise.
\end{itemize}
\end{definition}

\begin{definition}[Correctness]
The scheme is correct if honest computation yields correct decrypted results.
\begin{equation}
    \Pr\left[
    Dec_{sk}(c_y) = f(x)
    \;\middle|\;
    \begin{aligned}
        &(pk, sk) \leftarrow KGen(1^\lambda,f), \\
        &(c_x, \tau_x) \leftarrow Enc_{\text{key}}(x), \\
        &(c_y, \tau_y) \leftarrow Eval_{\text{key}}(c_x)
    \end{aligned}
    \right] = 1
\end{equation}
\end{definition}

\begin{definition}[Completeness]
The scheme is complete if the verify computation always accept an honest computation result.
\begin{equation}
    \Pr\left[
    \text{Verify}_{sk}(c_y, \tau_x, \tau_y) = 1
    \;\middle|\;
    \begin{aligned}
        &(pk, sk) \leftarrow \text{KGen}(1^\lambda,f), \\
        &(c_x, \tau_x) \leftarrow \text{Enc}_{\text{key}}(x), \\
        &(c_y, \tau_y) \leftarrow \text{Eval}_{\text{key}}(c_x)
    \end{aligned}
    \right] = 1
\end{equation}
\end{definition}

\begin{definition} [Soundness]
The scheme is sound if adversary cannot make the Verifier accept an incorrect or altered computation.
\begin{equation}
\Pr\left[
\begin{array}{c}
    \text{Verify}_{sk}(c_y, \tau_x, \tau_y) = 1 \\
    \land \\
    \text{Dec}_{sk}(c_y) \neq f(x)
\end{array}
\;\middle|\;
\begin{aligned}
    &(pk, sk) \leftarrow \text{KGen}(1^\lambda,f), \\
    &x \leftarrow A^{\text{OEnc},\text{ODec}}(pk), \\
    &(c_x, \tau_x) \leftarrow \text{Enc}_{\text{key}}(x), \\
    &(c_y, \tau_y) \leftarrow A^{\text{OEnc},\text{ODec}}(c_x, \tau_x)
\end{aligned}
\right] 
\end{equation}
\end{definition}

\begin{definition}[Security]
Formally, a scheme is secure if for any Probabilistic Polynomial Time (PPT) adversary $\mathcal{A}$ and any function $f$, the advantage $\text{Adv}^{\text{IND-CCA1}}_{\mathcal{A}}(\lambda) = 2\Pr[b = \hat{b}] - 1$ of the attacker in the following game is negligible in the security parameter $\lambda$:
\begin{center}
\textbf{IND-CCA1 for vFHE}
\end{center}
\begin{enumerate}
    \item $(pk, sk) \leftarrow \text{KGen}(1^\lambda, f)$
    \item $(m_0, m_1) \leftarrow \mathcal A^{{O}_{\text{Enc},\text{Dec}}}(1^\lambda, f, pk)$
    \item $(c^*, \tau^*) \leftarrow \text{Enc}_{pk}(m_b)$
    \item $\hat{b} \leftarrow \mathcal A^{{O}_{\text{Enc}}}(c^*)$
\end{enumerate}
\end{definition}
